A Comprehensive Survey of Unmanned Aerial Systems' Risks and Mitigation Strategies

In the last decade, the rapid growth of Unmanned Aircraft Systems (UAS) and Unmanned Aircraft Vehicles (UAV) in communication, defense, and transportation has increased. The application of UAS will continue to increase rapidly. This has led researchers to examine security vulnerabilities in various facets of UAS infrastructure and UAVs, which form a part of the UAS system to reinforce these critical systems. This survey summarizes the cybersecurity vulnerabilities in several phases of UAV deployment, the likelihood of each vulnerability's occurrence, the impact of attacks, and mitigation strategies that could be applied. We go beyond the state-of-the-art by taking a comprehensive approach to enhancing UAS security by performing an analysis of both UAS-specific and non-UAS-specific mitigation strategies that are applicable within the UAS domain to define the lessons learned. We also present relevant cybersecurity standards and their recommendations in the UAS context. Despite the significant literature in UAS security and the relevance of cyberphysical and networked systems security approaches from the past, which we identify in the survey, we find several critical research gaps that require further investigation. These form part of our discussions and recommendations for the future exploration by our research community.

==> UAV-Survey-NMSU/table/IgnoreInPageMitigationStandards.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly


\small
\begin{table}[cp]{|lll|}
\hline
\multicolumn{1}{|l|}{Attack Ref.} &
  \multicolumn{1}{l|}{Framework} &
  Mitigation Strategy \\ \hline
\multicolumn{3}{|c|}{UAV Hardware Attack} \\ \hline
\multicolumn{1}{|l|}{HW-S/*} &
  \multicolumn{1}{l|}{NISTIR 8323} & Identity verification, data verification, and validation of Positioning, Navigation, and Timing (PNT) components.\\ \hline
\multicolumn{1}{|l|}{HW-J/*} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  \begin{tabular}[c]{@{}l@{}}Software and hardware can be integrated into the system and critical infrastructure components to detect and \\ mitigate GNSS jamming and spoofing events and preserve data availability, continuity, and integrity.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{HW-FF} &
  \multicolumn{1}{l|}{NIST SP 800-193} &
  \begin{tabular}[c]{@{}l@{}}Firmware update images should be signed using an approved digital signature algorithm. The flash regions that \\ contain device firmware should be protected so that it is modifiable only through an authenticated update\\  mechanism to ensure the authenticity and integrity of the firmware update. The protection mechanisms shall \\ ensure that authenticated update mechanisms are not bypassed. If Critical Platform Firmware uses RAM for \\ temporary data storage, then this memory shall be protected from software running on the platform until the \\ data use is complete.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{HW-SCA} &
  \multicolumn{1}{l|}{NIST SP 800-161} &
  \begin{tabular}[c]{@{}l@{}}Establish an organization governance structure that meets ICT SCRM requirements and incorporates these \\ requirements into the organizational policies. Perform internal checks and balances to assure compliance \\ with security and quality requirements.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{UAV Software attack} \\ \hline
\multicolumn{1}{|l|}{SW-CI} &
  \multicolumn{1}{l|}{NIST SP 800-44} &
  \begin{tabular}[c]{@{}l@{}}Use secure programming practices and maintain secure configuration through application. Software, OS, web \\ servers, firewalls, packet filtering routers and proxy should be periodically scanned for vulnerability.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-DI} &
  \multicolumn{1}{l|}{NISTIR 7682} &
  \begin{tabular}[c]{@{}l@{}}Check the values in every field of a web form, looking for any characters that should not be in that type of data, \\ and looking for patterns that look like database commands. Monitor the logs of the database server, looking for \\ anomalous queries coming from the web server.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-FM} &
  \multicolumn{1}{l|}{NIST SP 800-147} &
  \begin{tabular}[c]{@{}l@{}}Use digital signatures for secure BIOS authentication. Authenticated BISO update mechanism should be an \\ exclusive mechanism for modification of system BIOS with proper authentication mechanism.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-BD} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}Use an uninterruptible power supply (UPS) that provides emergency power when there is a failure of the main \\ power source. The battery duration of most UPS is short but provides sufficient time to start a standby power \\ source such as a backup generator or properly shut down the system or perform emergency procedures.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-BO} &
  \multicolumn{1}{l|}{NIST SP 800-218} &
  \begin{tabular}[c]{@{}l@{}}Collect, protect, and regularly check provenance data for all software deployed in each environment, and \\ determine if any of the software or their dependencies have new known vulnerabilities.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{} &
  \begin{tabular}[c]{@{}l@{}}Review and approve all changes made to the code after the code has been automatically scanned for \\ vulnerabilities and any issues have been remediated. Periodically scan the software for buffer overflow flaws.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{} &
  Review and evaluate third-party software components in the context of their expected use. \\ \hline
\multicolumn{1}{|l|}{SW-MI} &
  \multicolumn{1}{l|}{NIST SP 800-83} &
  \begin{tabular}[c]{@{}l@{}}Scanning of media from outside of the organization for malware before they can be used. Restricting or \\ prohibiting the use of unnecessary software, such as user applications that are often used to transfer malware. \\ Using security automation technologies with OS and application configuration checklists to help administrators \\ secure hosts consistently and effectively.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-SCA} &
  \multicolumn{1}{l|}{NIST SP 800-161} &
  Similar to HW-SCA \\ \hline
\multicolumn{3}{|c|}{Ground Control System (GCS) Attack} \\ \hline
\multicolumn{1}{|l|}{GCS-RA} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}Employ automated mechanisms to facilitate the monitoring and control of remote access methods. Uses \\ encryption to protect the confidentiality of remote access sessions.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-FRQA} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Use antivirus software, intrusion prevention software, firewall, content filtering/inspection and application \\ whitelisting.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-DE} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  \begin{tabular}[c]{@{}l@{}}Minimize network exposure for all control system devices and/or systems and ensure that they are not \\ accessible from the Internet.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-PB} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}Use secure passwords and passphrase. Passwords should have minimum length and be followed by either \\ biometric authentication or two factor authentication. Stored passwords should be using an approved salted key \\ derivate function, preferably a keyed hash.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-RE} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}NIST CYBERSECURITY WHITE \\ PAPER on Mitigating the Risk of Software \\ Vulnerabilities by Adopting a Secure \\ Software Development Framework (SSDF)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Perform peer review of code, to check code for backdoors and other malicious content. Use automated tools to \\ identify and remediate documented and verified unsafe software practices on a continuous basis as \\ human-readable code is checked into the code repository.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-SE} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Avoid use of authenticators that present a risk of social engineering of third parties such as customer service \\ agents.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{Network Link Attack} \\ \hline
\multicolumn{1}{|l|}{NL-BH/GH} &
  \multicolumn{1}{l|}{NIST Special Publication 800-189} &
  \begin{tabular}[c]{@{}l@{}}Monitor the rate of queries/requests per source address and detect if an abnormally high volume of responses \\ is headed to the same destination (i.e., same IP address).\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-W} &
  \multicolumn{1}{l|}{NIST SP 800-189} &
  Similar to NL-BL/GH \\ \hline
\multicolumn{1}{|l|}{NL-Syb} &
  \multicolumn{1}{l|}{NISTIR 8301} &
  \begin{tabular}[c]{@{}l@{}}Sybil attack resistance is achieved, respectively, through built-in crypto economic incentives that enable \\ nodes to work together in zero-trust environments and through access control, wherein nodes must be \\ authorized by system owners or consortium members.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-Sink} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Different situations necessitate various combinations of eradication techniques. The most common tools for \\ eradication are antivirus software, spyware detection and removal utilities, and patch management software. \\ Providing instructions and software updates to users works in some cases.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-RFJa} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  Similar to HW-J/* \\ \hline
\multicolumn{1}{|l|}{NL-PBJa} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  Similar to HW-J/* \\ \hline
\multicolumn{1}{|l|}{NL-D} &
  \multicolumn{1}{l|}{NIST Interagency report 7316} &
  \begin{tabular}[c]{@{}l@{}}Use an access control list and access control matrix. Implement Separation of duty (SOD) where no user \\ should be given enough privileges to misuse the system.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PS/A} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Use antivirus, firewalls, application whitelisting sandboxing techniques. Eliminating unsecured file shares, \\ which are a common way for malware to spread.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PB} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Use an authenticator with high entropy authenticator secret. Store memorized secrets in a salted, hashed \\ form including a keyed hash.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PitM} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Communication between the claimant and verifier should be via an authenticated protected channel to \\ provide confidentiality of the authenticator output.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-CJ} &
  \multicolumn{1}{l|}{NIST SP 800-44} &
  Similar to SW-CI \\ \hline
\multicolumn{1}{|l|}{NL-M} &
  \multicolumn{1}{l|}{NIST SP 800-123} &
  \begin{tabular}[c]{@{}l@{}}Remove or disable unneeded default accounts, disable non interactive accounts. Create user groups, \\ configure automated time synchronization. Implement strong organization password policy.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-ReplayA} &
  \multicolumn{1}{l|}{NIST SP 800-63-3} &
  Use nonce that is used as challenge in challenge-response authentication protocol that are not repeated. \\ \hline
\multicolumn{1}{|l|}{NL-RelayA} &
  \multicolumn{1}{l|}{NIST CVE-2017-12819} &
  \begin{tabular}[c]{@{}l@{}}Locate control system networks and remote devices behind firewalls and isolate them from the business \\ network. When remote access is required, use secure methods, such as Virtual Private Networks (VPNs), \\ recognizing that VPNs may have vulnerabilities and should be updated to the most current version available.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-F} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}NISTIR 8397, NIST SP 800-95, \\ and NIST SP 800-53B\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}A type of dynamic analysis, known as fuzz testing, induces program failures by deliberately introducing \\ malformed or random data into software programs. Fuzz testing strategies are derived from the intended use \\ of applications and the functional and design specifications for the applications. To understand the scope of \\ dynamic code analysis and the assurance provided, organizations may also consider conducting code \\ coverage analysis and/or concordance analysis.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{Server Attack} \\ \hline
\multicolumn{1}{|l|}{SRV-DL} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  Similar to GCS-DE \\ \hline
\multicolumn{1}{|l|}{SRV-PIL} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63A} &
  \begin{tabular}[c]{@{}l@{}}Use a Credential Service Provider (CSP) that validates personal details in the evidence with the issuer \\ or other authoritative source. It verifies identity evidence and biometric of applicant against information \\ obtained from issuer or other authoritative source.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SRV-LL} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  Similar to GCS-DE \\ \hline
\end{table}


==> UAV-Survey-NMSU/table/Likelihood.tex <==
\begin{landscape}
\begin{table}[tbp]
\fontsize{7}{7}\selectfont
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}} &
  \multicolumn{21}{c|}{\begin{tabular}{c} UAS Phases of Operation \end{tabular}} \\ \cline{3-23} 
\multicolumn{2}{|l|}{} &
  \multicolumn{2}{l|}{ \begin{tabular}{c}Pre-Flight\\ /Mission \\ Planning \end{tabular} }  &
  
  \multicolumn{6}{l|}{ \begin{tabular}{c} Preparation   /System Checks \\ (applicable at almost all \\ phases of mission/flight) \end{tabular} }  &
  \multicolumn{5}{c|}{Launch} &
  \multicolumn{3}{l|}{ \begin{tabular}{c} Mission/ \\ Application \\ /Flight   \\ (Communication) \end{tabular} }  &
  \multicolumn{2}{l|}{ \begin{tabular}{c} Return \\ to Land \end{tabular} }  &
  \multicolumn{2}{l|}{ \begin{tabular}{c} Post- \\ Flight \end{tabular} }  &

  Others \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}{l} Attack \\ Reference \\ Number  \\ \\ \\  \end{tabular}} &
\multicolumn{1}{|l|}{\begin{tabular}{l} \\ Likelihood Legend: \\ A: Frequent\\ B: Probable\\ C: Remote \\ D: Extremely Remote\\ E: Extremely Improbable \\ \\ \\  \end{tabular}} &


%Likelihood Legend:\\Frequent (A): (Probability) ≥ 1 per 1,000\\ Probable (B): 1 per 1000 > (Probability) ≥ 1 per 100,000\\Remote (C): 1 per 100,000 > (Probability) ≥ 1 per 10,000,000\\Extremely Remote (D): 1 per 10,000,000 > (Probability) ≥ 1 per 1,000,000,000\\Extremely Improbable (E): 1 per 1,000,000,000 > (Probability) ≥ 1 per 10^14

  \rotatebox{90}{\parbox{3cm}{Flight Planning (both \\ for manual and autonomous)}}  & 
  \rotatebox{90}{\parbox{3cm}{Programming \\  flight (autonomous only)}}  & 
  
  \rotatebox{90}{\parbox{3cm}{Ground station}}  &
  \rotatebox{90}{\parbox{3cm}{Flight controls}}  &
  \rotatebox{90}{\parbox{3cm}{Data links}}  &
  \rotatebox{90}{\parbox{3cm}{GPS}}  &
  \rotatebox{90}{\parbox{3cm}{Sensors}}  &
  \rotatebox{90}{\parbox{3cm}{Power - battery/fuel}}  & 
  \rotatebox{90}{\parbox{3cm}{System checks   \\ (similar to those \\ noted above)}}  &
  \rotatebox{90}{\parbox{3cm}{Altimeter   verification}}  &
  \rotatebox{90}{\parbox{3cm}{Flight}}  &
  \rotatebox{90}{\parbox{3cm}{Manual}}  &
  \rotatebox{90}{\parbox{3cm}{Autonomous -  \\ Flight plan verification}}  &
  \rotatebox{90}{\parbox{3cm}{Data Relay -   \\ Telemetry}}  &
  \rotatebox{90}{\parbox{3cm}{Payload data -   \\ Video relay}}  &
  \rotatebox{90}{\parbox{3cm}{Payload data   -  \\ Sensor Information}}  &
  \rotatebox{90}{\parbox{3cm}{Manual}}  &
  \rotatebox{90}{\parbox{3cm}{Autonomous}}  &
  \rotatebox{90}{\parbox{3cm}{Ground Station}}  &
  \rotatebox{90}{\parbox{3cm}{Data Download}}  &
  \rotatebox{90}{\parbox{3cm}{Emergency \\ Procedures }}  
  \\ \hline
  \rowcolor{green}
\multicolumn{1}{|l|}{HW-ID} &
  UAV Hardware Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/GPS} &
  Spoofing - GPS &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/OS} &
  Spoofing - Other Sensors &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/ADSB-ID} &
  Spoofing - ADS-B,   Remote ID &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/A} &
  Spoofing - Actuator &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/GPS} &
  Jamming - GPS &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/OS} &
  Jamming - Other   Sensors &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/ADSB-ID} &
  Jamming - ADS-B,   Remote ID &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/A} &
  Jamming - Actuator &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-FF} &
  Firmware Flashing &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  C \\ \hline
  \rowcolor{lime}
\multicolumn{1}{|l|}{HW-SCA} &
  Supply Chain Attack &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
 \rowcolor{magenta}
\multicolumn{1}{|l|}{SW-ID} &
  UAV Software Attack &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \hline
    \rowcolor{pink}
\multicolumn{1}{|l|}{SW-CI} &
  Code Injection &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  E \\ \hline
   \rowcolor{pink}
\multicolumn{1}{|l|}{SW-DI} &
  Database Injection &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  C \\ \hline
   \rowcolor{pink}
\multicolumn{1}{|l|}{SW-FM} &
  Firmware Modification &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  D \\ \hline
%    \rowcolor{pink}
% \multicolumn{1}{|l|}{SW-BD} &
%   Battery Draining &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{D} &
%   \multicolumn{1}{l|}{E} &
%   \multicolumn{1}{l|}{E} &
%   D \\ \hline
   \rowcolor{pink}
\multicolumn{1}{|l|}{SW-BO} &
  Buffer Overflow &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  E \\ \hline
   \rowcolor{pink}
\multicolumn{1}{|l|}{SW-UA} &
  Unauthorized Access &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
 \rowcolor{pink}
\multicolumn{1}{|l|}{SW-MI} &
  Malware infection &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
   \rowcolor{pink}
\multicolumn{1}{|l|}{SW-SCA} &
  Supply Chain Attack &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
    \rowcolor{gray}
\multicolumn{1}{|l|}{GCS-ID} &
  Ground Control System   (GCS) Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-RA} &
  Remote access &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-FQA} &
  Forced quitting application &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-DE} &
  Data exfiltration &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-PB} &
  Password Breaking &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
 {\underline A} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-RE} &
  Reverse Engineering &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  D \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-SE} &
  Social Engineering &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline B} \\ \hline
  \rowcolor{orange}
\multicolumn{1}{|l|}{NL-ID} &
  Network Link Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-BH/GH} &
  Black Hole/Gray Hole &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline B} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-W} &
  Wormhole &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline B} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-Syb} &
  Sybil &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  D \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-Sink} &
  Sinkhole &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  E \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-RFJam} &
  Radio Frequency (RF)-based Jamming &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PBJam} &
  Protocol-based Jamming &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-D} &
  Deauthentication &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline B} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PS/A} &
  Packet Sniffing/Analysis &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PB} &
  Password Breaking &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PitM} &
  Person-In-The-Middle &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-CJ} &
  Command Injection &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-M} &
  Masquerading &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
 {\underline B} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-ReplayA} &
  Replay Attack &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
 {\underline A} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-RelayA} &
  Relay Attack &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  E \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-F} &
  Fuzzing &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
  \rowcolor{teal}
\multicolumn{1}{|l|}{SRV-ID} &
  Server Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{cyan}
\multicolumn{1}{|l|}{SRV-DL} &
  Data leakage &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
 {\underline A} \\ \hline
   \rowcolor{cyan}
\multicolumn{1}{|l|}{SRV-PIL} &
  Pilot identity leakage &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{C} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline B} &
  D \\ \hline
   \rowcolor{cyan}
\multicolumn{1}{|l|}{SRV-LL} &
  Location leakage &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{D} &
  \multicolumn{1}{l|}{\underline B} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{\underline A} &
  \multicolumn{1}{l|}{C} &
  C \\ \hline
\end{tabular}
%\vspace*{-0.95cm}
\caption{\label{tab:likelihood} UAV Likelihood Assessment Matrix.}
\end{table}
\end{landscape}



==> UAV-Survey-NMSU/table/LongMitigationInStandards.tex <==
\LTcapwidth=\textwidth
\begin{landscape}
\small
\begin{longtable}{|l|l|l|}
\caption{NIST standards help mitigate vulnerabilities in UAV Systems.\label{tab:MitigationStandards}} \\ \hline
\multicolumn{1}{|l|}{Attack Ref.} &
  \multicolumn{1}{l|}{Framework} &
 \multicolumn{1}{|c|}{ \textbf{ Mitigation Strategy}} \\ \hline
\multicolumn{3}{|c|}{UAV Hardware Attack} \\ \hline
\multicolumn{1}{|l|}{HW-S/*} &
  \multicolumn{1}{l|}{NISTIR 8323} & 
  Identity verification, data verification, and validation of Positioning, Navigation, and Timing (PNT) components.\\ \hline
\multicolumn{1}{|l|}{HW-J/*} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  \begin{tabular}[c]{@{}l@{}}Software and hardware can be integrated into the system and critical infrastructure components to detect and mitigate global \\ navigation satellite system (GNSS) jamming and spoofing events and preserve data availability, continuity, and integrity.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{HW-FF} &
  \multicolumn{1}{l|}{NIST SP 800-193} &
  \begin{tabular}[c]{@{}l@{}}Firmware update images should be signed using an approved digital signature algorithm. The flash regions that \\ contain device firmware should be protected so that it is modifiable only through an authenticated update\\  mechanism to ensure the authenticity and integrity of the firmware update. The protection mechanisms \\ ensure that authenticated update mechanisms are not bypassed. If Critical Platform Firmware uses RAM for \\ temporary data storage, then this memory is protected from software running on the platform until the \\ data use is complete.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{HW-SCA} &
  \multicolumn{1}{l|}{NIST SP 800-161} &
  \begin{tabular}[c]{@{}l@{}}Establish an organizational governance structure that meets ICT supply chain risk management (SCRM) requirements \\ and incorporates these requirements into the organizational policies. Perform internal checks and balances \\ to assure compliance with security and quality requirements.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{UAV Software Attack} \\ \hline
\multicolumn{1}{|l|}{SW-CI} &
  \multicolumn{1}{l|}{NIST SP 800-44} &
  \begin{tabular}[c]{@{}l@{}}Use secure programming practices and maintain secure configuration through the application. Software, OS, web \\ servers, firewalls, packet filtering routers, and proxy should be periodically scanned for vulnerability.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-DI} &
  \multicolumn{1}{l|}{NISTIR 7682} &
  \begin{tabular}[c]{@{}l@{}}Check the values in every field of a web form, validating for characters that should not be in that type of data, \\ and validating for patterns that look like database commands. Monitor the logs of the database server, and check for \\ anomalous queries coming from the web server.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-FM} &
  \multicolumn{1}{l|}{NIST SP 800-147} &
  \begin{tabular}[c]{@{}l@{}}Use digital signatures for secure BIOS authentication. Authenticated BIOS update mechanism should be an \\ exclusive mechanism for modification of system BIOS with proper authentication mechanism.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{} &
  \begin{tabular}[c]{@{}l@{}}Collect, protect, and regularly check provenance data for all software deployed in each environment, and \\ determine if any of the software or their dependencies have new known vulnerabilities.\end{tabular} \\ 
\multicolumn{1}{|l|}{SW-BO} &
  \multicolumn{1}{l|}{NIST SP 800-218} &
  \begin{tabular}[c]{@{}l@{}}Review and approve all changes made to the code after the code has been automatically scanned for \\ vulnerabilities and any issues have been remediated. Periodically scan the software for buffer overflow flaws.\end{tabular} \\ 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{} &
  Review and evaluate third-party software components in the context of their expected use. \\ \hline
\multicolumn{1}{|l|}{SW-UA} &
  \multicolumn{1}{l|}{NIST SP 800-63-B} &
  \begin{tabular}[c]{@{}l@{}} Using strong passwords and enabling MFA to reduce the risk of unauthorized access is essential. Managing authentication \\ credentials from registration to termination is vital to prevent unauthorized access. The document outlines three assurance \\ levels (IAL1, IAL2, and IAL3) based on the severity of the risk of unauthorized access and its potential impacts. These levels \\ help UAS operators match the level of identity assurance required to the sensitivity and risks associated with the UAS system.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-MI} &
  \multicolumn{1}{l|}{NIST SP 800-83} &
  \begin{tabular}[c]{@{}l@{}}Scanning of media from outside of the organization for malware before they can be used. Restricting or \\ prohibiting the use of unnecessary software, such as user applications that could potentially transfer malware. \\ Using security automation technologies with OS and application configuration checklists to help administrators \\ secure hosts consistently and effectively.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-SCA} &
  \multicolumn{1}{l|}{NIST SP 800-161} &
  Similar to HW-SCA \\ \hline
\multicolumn{3}{|c|}{Ground Control System (GCS) Attack} \\ \hline
\multicolumn{1}{|l|}{GCS-RA} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}Employ automated mechanisms to facilitate the monitoring and control of remote access methods. Uses \\ encryption to protect the confidentiality of remote access sessions.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-FQA} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Use antivirus software, intrusion prevention software, firewall, content filtering/inspection and application \\ whitelisting.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-DE} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  \begin{tabular}[c]{@{}l@{}}Minimize network exposure for all control system devices and/or systems and ensure that they are not \\ accessible from the internet.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-PB} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}Employ secure passwords and passphrases. Passwords should meet a specified minimum length and be \\ supplemented with either biometric authentication or two-factor authentication for enhanced security. When storing \\ passwords, it is advisable to use an approved salted key derivation function, ideally a keyed hash, to maintain the \\ integrity and safety of your credentials. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-RE} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}NIST Cybersecurity white \\ paper on Mitigating the Risk of Software \\ Vulnerabilities by Adopting a Secure \\ Software Development Framework (SSDF)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Perform peer review of code, to check code for backdoors and other malicious content. Use automated tools to \\ identify and remediate documented and verified unsafe software practices continuously as \\ human-readable code is checked into the code repository.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-SE} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Avoid the use of authenticators that present a risk of social engineering of third parties such as customer service \\ agents.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{Network Link Attack} \\ \hline
\multicolumn{1}{|l|}{NL-BH/GH} &
  \multicolumn{1}{l|}{NIST Special Publication 800-189} &
  \begin{tabular}[c]{@{}l@{}}Monitor the rate of queries/requests per source address and detect if an abnormally high volume of responses \\ is headed to the same destination (i.e., same IP address).\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-W} &
  \multicolumn{1}{l|}{NIST SP 800-189} &
  Similar to NL-BL/GH \\ \hline
\multicolumn{1}{|l|}{NL-Syb} &
  \multicolumn{1}{l|}{NISTIR 8301} &
  \begin{tabular}[c]{@{}l@{}}Sybil attack resistance is achieved, respectively, through built-in crypto-economic incentives that enable \\ nodes to work together in zero-trust environments and through access control, wherein nodes must be \\ authorized by system owners or consortium members.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-Sink} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Different situations necessitate various combinations of eradication techniques. The most common tools for \\ eradication are antivirus software, spyware detection and removal utilities, and patch management software. \\ Providing instructions and software updates to users works in some cases.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-RFJa} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  Similar to HW-J/* \\ \hline
\multicolumn{1}{|l|}{NL-PBJa} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  Similar to HW-J/* \\ \hline
\multicolumn{1}{|l|}{NL-D} &
  \multicolumn{1}{l|}{NIST Interagency report 7316} &
  \begin{tabular}[c]{@{}l@{}}Use an access control list and access control matrix. Implement separation of duty (SOD) where no user \\ should be given enough privileges to misuse the system.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PS/A} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Use antivirus, firewalls, application whitelisting sandboxing techniques. Eliminating unsecured file shares, \\ which are a common way for malware to spread.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PB} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Use an authenticator with high entropy authenticator secret. Store memorized secrets in a salted, hashed \\ form including a keyed hash.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PitM} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Communication between the claimant and verifier should be via an authenticated protected channel to \\ provide confidentiality of the authenticator output.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-CJ} &
  \multicolumn{1}{l|}{NIST SP 800-44} &
  Similar to SW-CI \\ \hline
\multicolumn{1}{|l|}{NL-M} &
  \multicolumn{1}{l|}{NIST SP 800-123} &
  \begin{tabular}[c]{@{}l@{}}Remove or disable unneeded default accounts, and disable non-interactive accounts. Create user groups, \\ configure automated time synchronization. Implement a strong organization password policy.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-ReplayA} &
  \multicolumn{1}{l|}{NIST SP 800-63-3} &
  Use nonce that is used as a challenge in challenge-response authentication protocols that are not repeated. \\ \hline
\multicolumn{1}{|l|}{NL-RelayA} &
  \multicolumn{1}{l|}{NIST CVE-2017-12819} &
  \begin{tabular}[c]{@{}l@{}}Locate control system networks and remote devices behind firewalls and isolate them from the business \\ network. When remote access is required, use secure methods, such as Virtual Private Networks (VPNs), \\ recognizing that VPNs may have vulnerabilities and should be updated to the most current version available.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-F} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}NISTIR 8397, NIST SP 800-95, \\ and NIST SP 800-53B\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}A type of dynamic analysis, known as fuzz testing, induces program failures by deliberately introducing \\ malformed or random data into software programs. Fuzz testing strategies are derived from the intended use \\ of applications and the functional and design specifications for the applications. To understand the scope of \\ dynamic code analysis and the assurance provided, organizations may also consider conducting code \\ coverage analysis and/or concordance analysis.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{Server Attack} \\ \hline
\multicolumn{1}{|l|}{SRV-DL} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  Similar to GCS-DE \\ \hline
\multicolumn{1}{|l|}{SRV-PIL} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63A} &
  \begin{tabular}[c]{@{}l@{}}Use a Credential Service Provider (CSP) that validates personal details in the evidence with the issuer \\ or other authoritative sources. It verifies the identity evidence and biometrics of the applicant against information \\ obtained from the issuer or other authoritative sources.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SRV-LL} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  Similar to GCS-DE \\ \hline
\end{longtable}
\end{landscape}


==> UAV-Survey-NMSU/table/MitigationStandardsReduced.tex <==
\LTcapwidth=\textwidth
\begin{landscape}
\small
\begin{longtable}{|l|l|l|}
\caption{NIST standards help mitigate vulnerabilities in UAV Systems (Contd.).\label{tab:MitigationStandardsReduced123}} \\ \hline
\endhead
\multicolumn{3}{r}{Continued on next page} \\ 
\endfoot
\endlastfoot
\hline
\multicolumn{1}{|l|} {\textbf{Attack Ref.}} &
  \multicolumn{1}{l|} {\textbf{Framework}} &
 \multicolumn{1}{|c|}{ \textbf{ Mitigation Strategy}} \\ \hline
\multicolumn{3}{|c|}{\textbf{UAV Hardware Attack}} \\ \hline
\multicolumn{1}{|l|}{HW-S/*} &
  \multicolumn{1}{l|}{NISTIR 8323} & 
  Validation of Positioning, Navigation, and Timing (PNT) components, identity, and data.\\ \hline
\multicolumn{1}{|l|}{HW-J/*} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  \begin{tabular}[c]{@{}l@{}}Global navigation satellite system (GNSS) jamming and spoofing events can be detected and mitigated, and data availability, \\ continuity, and integrity can be maintained by integrating hardware and software into essential infrastructure components.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{HW-FF} &
  \multicolumn{1}{l|}{NIST SP 800-193} &
  \begin{tabular}[c]{@{}l@{}}Digital signature algorithms that have been certified should be used to sign firmware update images. To guarantee \\ the integrity and authenticity of the firmware update, the flash regions containing the device firmware should be \\ secured such that only an authenticated update mechanism can modify it. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{HW-SCA} &
  \multicolumn{1}{l|}{NIST SP 800-161} &
  \begin{tabular}[c]{@{}l@{}}Incorporate ICT supply chain risk management (SCRM) requirements into organizational procedures. Maintain \\ compliance with security and quality requirements by conducting internal checks and balances.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{\textbf{UAV Software Attack} }\\ \hline
\multicolumn{1}{|l|}{SW-CI} &
  \multicolumn{1}{l|}{NIST SP 800-44} &
  \begin{tabular}[c]{@{}l@{}}Maintain secure configuration across the application and follow secure programming guidelines. Vulnerabilities should \\ be routinely checked in software, operating systems, web servers, firewalls, packet-filtering routers, and proxies.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-DI} &
  \multicolumn{1}{l|}{NISTIR 7682} &
  \begin{tabular}[c]{@{}l@{}}Verify all of the values in a web form, look for patterns that appear like database commands. Examine the database \\ server logs for unusual requests originating from the web server.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-FM} &
  \multicolumn{1}{l|}{NIST SP 800-147} &
  \begin{tabular}[c]{@{}l@{}}To ensure safe BIOS authentication, use digital signatures. BIOS update mechanism should be protected.\end{tabular} \\ \hline
% \multicolumn{1}{|l|}{} &
%   \multicolumn{1}{l|}{} &
%   \begin{tabular}[c]{@{}l@{}}Gather and safeguard provenance data for all software utilized in every environment. It is necessary to assess \\ if any of the software or its dependencies have new known vulnerabilities.\end{tabular} \\ 
% \multicolumn{1}{|l|}{SW-BO} &
%   \multicolumn{1}{l|}{NIST SP 800-218} &
%   \begin{tabular}[c]{@{}l@{}} Automatically check code for vulnerabilities. Check for buffer overflow vulnerabilities in the program regularly.\end{tabular} \\ 
% \multicolumn{1}{|l|}{} &
%   \multicolumn{1}{l|}{} &
%   Examine and assess third-party software components according to the intended use. \\ \hline
\multicolumn{1}{|l|}{SW-BO} &
  \multicolumn{1}{l|}{NIST SP 800-218} &
  \begin{tabular}[c]{@{}l@{}} Gather and safeguard provenance data for all software utilized in every environment. It is necessary to assess if any of the \\ software or its dependencies have new known vulnerabilities. Automatically check code for vulnerabilities. Check for buffer \\ overflow vulnerabilities in the program regularly. Examine and assess third-party software components according to the \\ intended use. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-UA} &
  \multicolumn{1}{l|}{NIST SP 800-63-B} &
  \begin{tabular}[c]{@{}l@{}} Use strong passwords and enable multi-factor authentication (MFA) to minimize the risk of unauthorized access. \\ Proper management of authentication credentials, from the moment of registration to termination, is essential to \\ prevent unauthorized access. The document outlines three assurance levels (IAL1, IAL2, and IAL3) based \\ on the severity of the risk of unauthorized access and its potential impacts. These levels help UAS operators to determine \\ the level of identity assurance required, depending on the sensitivity and risks associated with the UAS system.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-MI} &
  \multicolumn{1}{l|}{NIST SP 800-83} &
  \begin{tabular}[c]{@{}l@{}}External media should first be scanned for malware before being utilized. Limiting or prohibiting the usage of unneeded \\ software, like user applications that could introduce viruses, administrators can safeguard hosts reliably by combining security \\ automation technologies.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SW-SCA} &
  \multicolumn{1}{l|}{NIST SP 800-161} &
  Similar to HW-SCA \\ \hline
\multicolumn{3}{|c|}{\textbf{Ground Control System (GCS) Attack}} \\ \hline
\multicolumn{1}{|l|}{GCS-RA} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}Remote access session's privacy can be protected using encryption.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-FQA} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Use application whitelisting, firewalls, intrusion prevention systems, antivirus software, and content filtering/inspection.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-DE} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  \begin{tabular}[c]{@{}l@{}}Minimize network exposure for all control system devices.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-PB} &
  \multicolumn{1}{l|}{NIST SP 800-53} &
  \begin{tabular}[c]{@{}l@{}}For maximum security, passwords should be at least a certain length and should be reinforced with two-factor or biometric \\ authentication. To ensure the security and integrity of credentials, it is recommended to utilize a keyed hash or another \\ authorized salted key derivation function when saving passwords. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-RE} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}NIST Cybersecurity white \\ paper on Mitigating the Risk of Software \\ Vulnerabilities by Adopting a Secure \\ Software Development Framework (SSDF)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Conduct code peer review to ensure that it is free of malicious content and backdoors. A human-readable code that is \\ checked into the code repository can be continuously monitored using automated technology to discover dangerous \\ software practices. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{GCS-SE} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Avoid using authenticators that can be socially engineered by third parties, such as customer service agents.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{\textbf{Network Link Attack}} \\ \hline
\multicolumn{1}{|l|}{NL-BH/GH} &
  \multicolumn{1}{l|}{NIST Special Publication 800-189} &
  \begin{tabular}[c]{@{}l@{}}Observe how many requests or queries are made for each source address and keep a note whether an abnormally large \\ number of answers are being delivered to the same IP address.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-W} &
  \multicolumn{1}{l|}{NIST SP 800-189} &
  Similar to NL-BL/GH \\ \hline
\multicolumn{1}{|l|}{NL-Syb} &
  \multicolumn{1}{l|}{NISTIR 8301} &
  \begin{tabular}[c]{@{}l@{}}Sybil attack resistance is attained by access control, which requires nodes to be approved by consortium members or \\ system owners, and by built-in crypto-economic incentives that allow nodes to cooperate in zero-trust environments.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-Sink} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Different combinations of eradication procedures are required in different conditions. Patch management software, \\ spyware detection, and antivirus software are popular eradication tools. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-RFJa} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  Similar to HW-J/* \\ \hline
\multicolumn{1}{|l|}{NL-PBJa} &
  \multicolumn{1}{l|}{NISTIR 8323} &
  Similar to HW-J/* \\ \hline
\multicolumn{1}{|l|}{NL-D} &
  \multicolumn{1}{l|}{NIST Interagency report 7316} &
  \begin{tabular}[c]{@{}l@{}}Employ an access control matrix and an access control list. Use separation of duties (SOD), which states that no user \\ should have adequate access to the system to abuse it.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PS/A} &
  \multicolumn{1}{l|}{NIST Special Publication 800-83} &
  \begin{tabular}[c]{@{}l@{}}Employ sandboxing techniques, firewalls, and antivirus software. Avoid insecure file sharing, which is a popular \\ conduit for malware distribution.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-PB} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}Use authenticators with a high entropy. Passwords should be kept in a salted and hashed format with a keyed hash.\end{tabular} \\ \hline
  %%%%%%%%%%%%%
\multicolumn{1}{|l|}{NL-PitM} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63B} &
  \begin{tabular}[c]{@{}l@{}}To guarantee the privacy of the authenticator output, communication between the claimant and the verifier must take \\ place over a protected, authenticated channel.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-CJ} &
  \multicolumn{1}{l|}{NIST SP 800-44} &
  Similar to SW-CI \\ \hline
\multicolumn{1}{|l|}{NL-M} &
  \multicolumn{1}{l|}{NIST SP 800-123} &
  \begin{tabular}[c]{@{}l@{}}Disable inactive accounts, remove unnecessary default accounts. Establish user groups and set up automatic time \\ synchronization. Establish a robust password policy.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-ReplayA} &
  \multicolumn{1}{l|}{NIST SP 800-63-3} &
Employ a nonce that is used as a challenge in one-time challenge-response authentication methods. \\ \hline
\multicolumn{1}{|l|}{NL-RelayA} &
  \multicolumn{1}{l|}{NIST CVE-2017-12819} &
  \begin{tabular}[c]{@{}l@{}}To ensure security, it is recommended that the control system networks and remote devices be located behind firewalls \\ and kept separate from the business network. In situations where remote access is necessary, secure methods such as \\ Virtual Private Networks (VPNs) should be used. VPNs may have vulnerabilities and should be updated to the latest \\ version when available.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{NL-F} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}NISTIR 8397, NIST SP 800-95, \\ and NIST SP 800-53B\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Fuzz testing is a technique for dynamic software analysis. It involves inserting faulty data to identify program failures. \\ To better understand dynamic code analysis, organizations can use the test to perform code coverage and concordance \\ analysis.\end{tabular} \\ \hline
\multicolumn{3}{|c|}{\textbf{Server Attack}} \\ \hline
\multicolumn{1}{|l|}{SRV-DL} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  Similar to GCS-DE \\ \hline
\multicolumn{1}{|l|}{SRV-PIL} &
  \multicolumn{1}{l|}{NIST Special Publication 800-63A} &
  \begin{tabular}[c]{@{}l@{}}Use Credential Service Provider (CSP) along with biometric data.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{SRV-LL} &
  \multicolumn{1}{l|}{ICS Advisory (ICSA-19-015-01)} &
  Similar to GCS-DE \\ \hline
\end{longtable}
\end{landscape}


==> UAV-Survey-NMSU/table/Severity.tex <==
\begin{landscape}
\begin{table}[!htbp]
%\tiny
\fontsize{7}{7}\selectfont
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}} &
  \multicolumn{21}{c|}{\begin{tabular}{c} UAS Phases of Operation \end{tabular}} \\ \cline{3-23} 
  \multicolumn{2}{|l|}{} &
  \multicolumn{2}{l|}{ \begin{tabular}{c}Pre-Flight\\ /Mission \\ Planning \end{tabular} }  &
  
  \multicolumn{6}{l|}{ \begin{tabular}{c} Preparation   /System Checks \\ (applicable at almost all \\ phases of mission/flight) \end{tabular} }  &
  \multicolumn{5}{c|}{Launch} &
  \multicolumn{3}{l|}{ \begin{tabular}{c} Mission/ \\ Application \\ /Flight   \\ (Communication) \end{tabular} }  &
  \multicolumn{2}{l|}{ \begin{tabular}{c} Return \\ to Land \end{tabular} }  &
  \multicolumn{2}{l|}{ \begin{tabular}{c} Post- \\ Flight \end{tabular} }  &

  Others \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}{l} Attack \\ Reference \\ Number  \\ \\ \\ \end{tabular}} &
\multicolumn{1}{|l|}{\begin{tabular}{l} \\ Severity Legend: \\ 5: Minimal\\ 4: Minor\\ 3: Major \\ 2: Hazardous\\ 1: Catastrophic  \\ \\ \\ \end{tabular}} &
  \rotatebox{90}{\parbox{3cm}{Flight Planning (both \\ for manual and autonomous)}}  & 
  \rotatebox{90}{\parbox{3cm}{Programming \\  flight (autonomous only)}}  & 
  
  \rotatebox{90}{\parbox{3cm}{Ground station}}  &
  \rotatebox{90}{\parbox{3cm}{Flight controls}}  &
  \rotatebox{90}{\parbox{3cm}{Data links}}  &
  \rotatebox{90}{\parbox{3cm}{GPS}}  &
  \rotatebox{90}{\parbox{3cm}{Sensors}}  &
  \rotatebox{90}{\parbox{3cm}{Power - battery/fuel}}  & 
  \rotatebox{90}{\parbox{3cm}{System checks   \\ (similar to those \\ noted above)}}  &
  \rotatebox{90}{\parbox{3cm}{Altimeter   verification}}  &
  \rotatebox{90}{\parbox{3cm}{Flight}}  &
  \rotatebox{90}{\parbox{3cm}{Manual}}  &
  \rotatebox{90}{\parbox{3cm}{Autonomous -  \\ Flight plan verification}}  &
  \rotatebox{90}{\parbox{3cm}{Data Relay -   \\ Telemetry}}  &
  \rotatebox{90}{\parbox{3cm}{Payload data -   \\ Video relay}}  &
  \rotatebox{90}{\parbox{3cm}{Payload data   -  \\ Sensor Information}}  &
  \rotatebox{90}{\parbox{3cm}{Manual}}  &
  \rotatebox{90}{\parbox{3cm}{Autonomous}}  &
  \rotatebox{90}{\parbox{3cm}{Ground Station}}  &
  \rotatebox{90}{\parbox{3cm}{Data Download}}  &
  \rotatebox{90}{\parbox{3cm}{Emergency \\ Procedures }}  
  \\ \hline
  \rowcolor{green}
\multicolumn{1}{|l|}{HW-ID} &
  UAV Hardware Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/GPS} &
  Spoofing - GPS &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/OS} &
  Spoofing - Other Sensors &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/ADSB-ID} &
  Spoofing - ADS-B,   Remote ID &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  4 \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-S/A} &
  Spoofing - Actuator &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/GPS} &
  Jamming - GPS &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/OS} &
  Jamming - Other   Sensors &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/ADSB-ID} &
  Jamming - ADS-B,   Remote ID &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  4 \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-J/A} &
  Jamming - Actuator &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-FF} &
  Firmware Flashing &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  {\underline 1} \\ \hline
   \rowcolor{lime}
\multicolumn{1}{|l|}{HW-SCA} &
  Supply Chain Attack &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 2} \\ \hline
   \rowcolor{magenta}
\multicolumn{1}{|l|}{SW-ID} &
  UAV Software Attack &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
   \\ \hline
   \rowcolor{pink}
\multicolumn{1}{|l|}{SW-CI} &
  Code Injection &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{pink}
\multicolumn{1}{|l|}{SW-DI} &
  Database Injection &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{pink}
\multicolumn{1}{|l|}{SW-FM} &
  Firmware Modification &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
%   \rowcolor{pink}
% \multicolumn{1}{|l|}{SW-BD} &
%   Battery Draining &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   \multicolumn{1}{l|}{5} &
%   4 \\ \hline
  \rowcolor{pink}
\multicolumn{1}{|l|}{SW-BO} &
  Buffer Overflow &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 2} \\ \hline
  \rowcolor{pink}
\multicolumn{1}{|l|}{SW-UA} &
  Unauthorized Access &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  {\underline 1} \\ \hline
  \rowcolor{pink}
\multicolumn{1}{|l|}{SW-MI} &
  Malware infection &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  {\underline 1} \\ \hline
  \rowcolor{pink}
\multicolumn{1}{|l|}{SW-SCA} &
  Supply Chain Attack &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 2} \\ \hline
  \rowcolor{gray}
\multicolumn{1}{|l|}{GCS-ID} &
  Ground Control System   (GCS) Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-RA} &
  Remote access &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  3 \\ \hline
  \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-FQA} &
  Forced quitting application &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-DE} &
  Data exfiltration &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  5 \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-PB} &
  Password Breaking &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-RE} &
  Reverse Engineering &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{lightgray}
\multicolumn{1}{|l|}{GCS-SE} &
  Social Engineering &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
   \rowcolor{orange}
\multicolumn{1}{|l|}{NL-ID} &
  Network Link Attack &
  \multicolumn{21}{l|}{} \\ \hline
   \rowcolor{brown}
\multicolumn{1}{|l|}{NL-BH/GH} &
  Black Hole/Gray Hole &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-W} &
  Wormhole &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-Syb} &
  Sybil &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 2} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-Sink} &
  Sinkhole &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 2} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-RFJam} &
  Radio Frequency (RF)-based Jamming &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PBJam} &
  Protocol-based Jamming &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-D} &
  Deauthentication &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PS/A} &
  Packet Sniffing/Analysis &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  5 \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PB} &
  Password Breaking &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-PitM} &
  Person-In-The-Middle &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  5 \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-CJ} &
  Command Injection &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-M} &
  Masquerading &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 2} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-ReplayA} &
  Replay Attack &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-RelayA} &
  Relay Attack &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{brown}
\multicolumn{1}{|l|}{NL-F} &
  Fuzzing &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{\underline 1} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  {\underline 1} \\ \hline
  \rowcolor{teal}
\multicolumn{1}{|l|}{SRV-ID} &
  Server Attack &
  \multicolumn{21}{l|}{} \\ \hline
  \rowcolor{cyan}
\multicolumn{1}{|l|}{SRV-DL} &
  Data leakage &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  5 \\ \hline
  \rowcolor{cyan}
\multicolumn{1}{|l|}{SRV-PIL} &
  Pilot identity leakage &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  5 \\ \hline
  \rowcolor{cyan}
\multicolumn{1}{|l|}{SRV-LL} &
  Location leakage &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{4} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{3} &
  \multicolumn{1}{l|}{5} &
  \multicolumn{1}{l|}{5} &
  3 \\ \hline
\end{tabular}

\caption{\label{tab:severity}  UAV Severity Assessment Matrix.}
\end{table}
\end{landscape}


